CrashScope: A Practical Tool for Automated Testing of Android Applications

Unique challenges arise when testing mobile applications due to their prevailing event-driven nature and complex contextual features (e.g. sensors, notifications). Current automated input generation approaches for Android apps are typically not practical for developers to use due to required instrumentation or platform dependence and generally do not effectively exercise contextual features. To better support developers in mobile testing tasks, in this demo we present a novel, automated tool called CrashScope. This tool explores a given Android app using systematic input generation, according to several strategies informed by static and dynamic analyses, with the intrinsic goal of triggering crashes. When a crash is detected, CrashScope generates an augmented crash report containing screenshots, detailed crash reproduction steps, the captured exception stack trace, and a fully replayable script that automatically reproduces the crash on a target device(s). Results of preliminary studies show that CrashScope is able to uncover about as many crashes as other state of the art tools, while providing detailed useful crash reports and test scripts to developers. Website: www.crashscope-android.com/crashscope-home Video url: https://youtu.be/ii6S1JF6xDw

==> macro.tex <==


\usepackage{amssymb}
\usepackage{ifthen}

\makeatletter

% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}


\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }



\newcommand\MARTY[1]{\nb{MARTY}{#1}}
\newcommand\KEVIN[1]{\nb{KEVIN}{#1}}
\newcommand\DENYS[1]{\nb{DENYS}{#1}}
\newcommand\MARIO[1]{\textcolor{red}{\nb{MARIO}{#1}}}
\newcommand\CARLOS[1]{\nb{CARLOS}{#1}}
\newcommand\CHRIS[1]{\nb{CHRIS}{#1}}

\newcommand\NEW[1]{\nb{NEW}{#1}}






==> related-works.tex <==
% !TEX root = main.tex
\vspace{-0.15cm}
In this section, we overview the current landscape of automated testing and input generation tools for Android, discussing limitations of these approaches while illustrating \CrashScopes novelty in context. %, differentiating the novelty of our work in these contexts.
 Several approaches for detecting and reproducing crashes are available in literature \cite{Csallner:SPE2004,Pacheco:ECOOP2005,Csallner:TSEM2008,Pacheco:ICSE2007,Lohman:ICAC2005,Dang:ICSE2012,42Wu:ISSTA2014,8Zhou:ICSE12,Zeller:2005,Zeller:FSE2002,Yoo:TSEM2013,Seo:ASE2012,Liu:FSE2013,46Kim:DSN2011,26Jin:ISSTA13,18Jin:ICSE12}%\DENYS{[REFs from our CRASHDROID paper; all the refs between 24-43, do not include 29-31 and 41]}
 ; however, we forgo discussion of these approaches, as they are not presented in the context of mobile apps, and hence do not consider the unique associated challenges.

%\subsection{Types of Android Application Crashes}
%\MARIO{Kevin please show both dialogs (Fig 1) in a row to save space }

%There are two major types of Android application crashes which we will briefly outline in this section.  
%Android apps are written mainly in Java and follow an event-driven design paradigm.  This means that the event-flow of an app is highly dependent upon user input to trigger actions and transitions between different ``screens" (i.e., dialogs and activities).  This inherent nature places practical restrictions on the amount of computational work that can be done on the main thread of a particular screen in the application.  The ``UI thread" is responsible for processing user input, and thus if the app blocks on some action that is computationally expensive or I/O intensive, the app can become unresponsive from the users' point of view \cite{android-responsiveness,Liu:ICSE14}.  This leads to the first type of Android app crash, known as an \textit{Application Not Responding} (ANR) (Figure \ref{crashes}-A). %which is recognized as a dialog notifying the user that the application is unresponsive.  
%A second common type of crash occurs when an app throws an uncaught, fatal exception.  In this situation, the system displays a dialog  (see Figure \ref{crashes}-B) and is also known as a force close of the application.  As we discuss later, force closes of an app manifest much more frequently than the ANRs. \KEVIN{We can probably cut this section if we need space.}

%\begin{figure}[b]
%\centering
%\includegraphics[scale=0.4]{img/android-crashes.pdf}
%\caption{Examples of dialogs for a crashing Android app}
%\label{crashes}
%\end{figure}
\vspace{-0.15cm}
\subsection{Input Generation \& Testing Tools for Mobile Apps}
\vspace{-0.1cm}
%Based on the competitive nature of the app store and the damaging nature of application crashes, there is clear motivation for developers to thoroughly test their applications for crashes and other faults to ensure the highest quality software product is released to the public for either an initial release or subsequent updates.  

%The complications introduced by the nature of mobile apps can prohibit developers from effectively carrying out maintenance tasks.  This fact has lead to research regarding automated tools for Android input generation with goals of increasing testing code coverage and app fault discovery.  There are several intellectual and technical challenges that must be met for tools aiming to automatically and effectively discover and report faults in mobile apps, some of which have been outlined in \cite{Choudhary:ARCX15}:

%\begin{enumerate}
%\item{\textit{The tool's exploration heuristic must be effective at uncovering application faults.}}
%\item{\textit{The tool should be able to automatically produce replayable scenarios/scripts for fault reproduction.}}
%\item{\textit{The tool should present a detailed readable report to the developer outlining reproduction steps and the relevant application event-flow.}}
%\item{\textit{The tool should be able to operate on several different hardware and phone models and emulators supporting popular and widely used versions of the Android OS.}}
%\item{\textit{The tool should be easy to use (black box), requiring as input only the testing parameters and the application .apk file or source code, not requiring expensive and fault prone instrumentation of the OS or application source code}}
%\end{enumerate}

\begin{table*}[tb]
\vspace{-0.6cm}
\centering
\caption{An Overview of features in automated testing approaches for mobile applications
%\textnormal{(N/A means either means that the feature category does not apply to the testing approach, or that it could not be inferred from the implementation details given by the tool's corresponding paper) *This table expands upon the categorization presented in \cite{Choudhary:ASE15}}
}
\vspace{-0.3cm}
\label{fig:android_approaches}
\scriptsize
\begin{tabular}{| p{65pt} | p{50pt} | p{70pt} | p{69pt} | p{37pt} | p{42pt} | p{39pt} | p{44pt} | p{45pt} |}
\hline
\textbf{Tool Name}& \textbf{Instrumentation} & \textbf{GUI Exploration} & \textbf{Types of Events} & \textbf{Crash Resilient}  & \textbf{Replayable Test Cases} & \textbf{NL Crash Reports} & \textbf{Emulators, Devices} \\ \hline

Dynodroid\cite{Machiry:FSE13}  & Yes & Guided/Random & System, GUI, Text  & Yes & No & No & No  \\ \hline

EvoDroid \cite{Mahmood:FSE14}  & No & System/Evo & GUI & No & No & No  & N/A \\ \hline

\textit{Android}Ripper \cite{Amalfitano:ASE12} & Yes & Systematic & GUI, Text & No & No & No  & N/A \\ \hline 

MobiGUItar \cite{Amalfitano:IEEE14}  & Yes & Model-Based & GUI, Text & No & Yes & No  & N/A\\ \hline

A$^3$E Depth-First \cite{Azim:OOPSLA13}  & Yes & Systematic  & GUI  & No & No & No  & Yes \\ \hline

A$^3$E Targeted\cite{Azim:OOPSLA13}  & Yes & Model-Based  & GUI & No & No & No &  Yes \\ \hline

Swifthand \cite{Choi:OOPSLA13}  & Yes & Model-Based & GUI, Text & N/A & No & No  & Yes   \\ \hline

PUMA \cite{Hao:Mobisys14}  & Yes & Programmable & System, GUI, Text & N/A & No & No  & Yes \\ \hline

ACTEve \cite{Anand:FSE12}  & Yes & Systematic & GUI & N/A & No & No  & Yes  \\ \hline

VANARSena \cite{Ravindranath:Mobisys2014}  & Yes & Random & System, GUI, Text & Yes & Yes & No  & N/A  \\ \hline

Thor \cite{Adamsen:ISSTA2015}  & Yes & Test Cases & Test Case Events & N/A & N/A & No  & No  \\ \hline

QUANTUM \cite{Zaeem:ICST2014}  & Yes & Model-Based & System, GUI & N/A & Yes & No & N/A  \\ \hline

AppDoctor \cite{Hu:ESYS14} & Yes & Multiple & System, GUI$^2$, Text & Yes & Yes & No  & N/A  \\ \hline

ORBIT \cite{Yang:FASE13}  & No & Model-Based & GUI & N/A & No & No  & N/A  \\ \hline

SPAG-C \cite{Lin:TSE14}  & No & Record/Replay & GUI & N/A & N/A & No  & No  \\ \hline

JPF-Android \cite{vanderMerwe:SEN2014}  & No & Scripting & GUI & N/A & Yes & No  & N/A  \\ \hline

MonkeyLab\cite{Linares:MSR15} & No & Model-based & GUI, Text & No & Yes & No  & Yes \\ \hline

CrashDroid \cite{White:ICPC15} & No & Manual Rec/Replay & GUI, Text & Manual & Yes & Yes  &  Yes \\ \hline

SIG-Droid \cite{Mirzaei:ISSRE15} & No & Symbolic & GUI, Text & N/A & Yes & No & N/A  \\ \hline

\textbf{CrashScope}  & \textbf{No} & \textbf{Systematic} & \textbf{GUI, Text, System} & \textbf{Yes} & \textbf{Yes} & \textbf{Yes} & \textbf{Yes}  \\ \hline
\end{tabular}
 %$^1$ It was unclear whether some approaches implemented User Text Input or System-level Contextual events. $^2$  App Doctor uses approximate execution and then replays traces to filter out false positives. $^3$ Contextual system features can only be exercised in an emulator.   
\vspace{-0.7cm}
\end{table*}

	%Several recent research approaches have aimed to improve solutions for testing and automatic input generation for mobile apps. We survey the general features of several such testing and input generation tools in Table \ref{fig:android_approaches}. 
	Approaches for automated input generation can be broadly grouped into three major categories \cite{Choudhary:ASE15}: \textit{random-based input generation}\cite{Machiry:FSE13,android-monkey,intent-fuzzer,Sasnauskas:WODA14,Ye:MoMM13}, %which generate random events to be executed on a target app; 
\textit{systematic input generation}\cite{Azim:OOPSLA13,Anand:FSE12,Amalfitano:ASE12}, % which systematically test the app using a predefined heuristic
and \textit{model-based testing}\cite{Amalfitano:ASE12,Yang:FASE13,Azim:OOPSLA13,Choi:OOPSLA13,Hao:Mobisys14,Zaeem:ICST2014}.
% which generate events according to a pre-existing or dynamically generated model of the app.
  We outline some features of several mobile testing and input generation tools in Table \ref{fig:android_approaches}. 
%DENYS: COMMENTED OUT FOR NOW, since it is repetitive info.
%Other recent  approaches in testing mobile apps listed in the Table \ref{fig:android_approaches} attempt to solve specific testing problems such as the generation of test oracles, the creation of extensible testing frameworks, or stress testing apps in adverse contextual conditions.  In this section we briefly survey the tools listed in Table \ref{fig:android_approaches} and discuss the current general limitations of these approaches.
	%\DENYS{Perhaps put the lists of citations for the papers in each category here}
	%We briefly survey the approaches that most closely mimic \CrashScope in terms of functionality.   

%\textbf{Dynodroid} \cite{} developed by Machinery et. al, is an augmented variation of random input generation that maintains a history of how often different events are executed in a context sensitive manner that tracks relevant events throughout the execution.

%\textbf{VANARSena }\cite{}  The major goal of the VanarSena framework is to implement a scalable easy to use system that test mobile apps for common externally-inducible faults as thoroughly as possible.  This approach requires binary instrumentation in order to automate the UI exploration and implement a module that the authors call the Fault Inducer that is able to inject adverse contextual conditions that can occur during the course of a user interacting with an application.   This approach does generate crash reports with a stack trace and a list of user interactions.  The authors give no direct details regarding the exact information in the crash reports, however, the paper seems to suggest that they take the form of crash logs rather than what would be considered crash reports.

\textbf{Random-Based Input Generation} techniques rely on choosing arbitrary GUI or contextual events; they can adapt such a strategy through biasing the selection with the frequency of past events and purposefully select those previously un-exercised. Dynodroid \cite{Machiry:FSE13} introduces such an approach by maintaining a history of event execution frequencies in a context-sensitive manner that tracks relevant events throughout the execution.   %While Dynodroid can exercise a diverse set of events, it is unable to generate detailed fault reports as \CrashScope does. 
Intent Fuzzer \cite{Sasnauskas:WODA14} generates intents to test apps by taking into consideration information extracted in an offline static analysis phase. However, it does not easily scale for large apps due to the number of paths that need to be stored in memory for processing, and only tests app intents. VanarSena \cite{Ravindranath:Mobisys2014} is a tool for Windows Phone that instruments app binaries in order to test apps for externally-inducible faults using random exploration and the injection of adverse contextual conditions.  VanarSena  is capable of generating crash reports containing a stack trace and exception. Compared to VanarSena, \CrashScopesp does not require any type of instrumentation and is able to generate more detailed crash reports that include screenshots, natural language reproduction steps, and replayable scripts.

%\textbf{Evodroid }\cite{} This paper presents a testing approach that relies on an evolutionary genetic algorithm in order to support the testing of Android apps.  EvoDroid extracts two models 1) an Interface Model, which is extracted by parsing the Android Manifest to discover all of the activities in an app and the corresponding layout files in order to extract all of the statically declared GUI elements in an app, and 2) a Call-Graph-Model, which is extracted statically using a tool called MoDisco, which the authors extended to generate fully connected graphs for Android.  To generate test cases, EvoDroid starts at the root of the Connected Call-Graph and generates sequences of events with the goal of reaching the leaf nodes to improve coverage.  EvoDroid breaks each path in the connected call-graph into segments and runs an evolutionary algorithm on each segment in order to maximize code coverage.  

%\textbf{\textit{Android}Ripper} \cite{} This approach is a "ripping" technique that exercises an app's GUI in a structured manner.  This is one of the earliest approaches for the automated testing and input generation of Android apps.  AndroidRipper dynamically analyzes an app?s GUI with the aim of obtaining a sequence of events fire-able through an app?s GUI.  AndroidRipper is designed based on executing tasks in a task list, starting with the tasks that are feasible in the Main Activity of an App, the task list is iteratively updated with new tasks as execution progresses.  This is a systematic exploration approach. 

%\textbf{A$^3$E Depth-First} \cite{} This approach leverages static bytecode, taint-style, dataflow analysis in order to construct a high-level control flow-graph that captures legal transitions between app screens (activities).  This tool is able to extract a Static Activity Transition Graph (SATG) through static taint analysis. From this model the authors implement two exploration strategies, Targeted Exploration and Depth-First Exploration.  The Depth First version of this tool exercises fireable elements in the GUI hierarchy on each screen in a depth first manner. The framework for this tool is built on top of Robotium and is not capable of executing system level events.

%%\textbf{ACTEve }\cite{} This is an approach based on concolic testing of smartphone apps that helps to alleviate the path explosion problem by checking a condition on program execution that identifies subsumption between different event sequences.  This approach symbolically tracks events from the point where they originate to the point where they are handled.  Because of this it requires instrumentation of the Android SDK and the app under test.  This approach is only for GUI-driven testing and aims at generating single events and event streams.  The authors offer a formal proof in the paper to show that their approach covers the same number of program branches and hence the same number of program states as standard concolic execution.

\textbf{Systematic Input Generation} approaches execute input events according to a pre-defined heuristic such as Breadth or Depth First Search (BFS/DFS).  %\MARIO{\textcolor{red}{Evodroid can not be in this category. There should be a category for hydrid approaches. Evodroid is not systematic input generation}}
For instance, \textit{Android}Ripper dynamically analyzes an app's GUI with the aim of obtaining a fireable sequence of events.  It then extracts task lists according to the GUI hierarchy of an app and systematically executes the events in the generated lists.  %\CrashScopesp builds upon the GUI-ripping technique introduced by \textit{Android}Ripper and implements different strategies for generating text input and exercising contextual events.  
A$^3$E \cite{Azim:OOPSLA13} leverages static bytecode, taint-style, dataflow analysis in order to construct a high-level control flow-graph that captures allowable transitions between app screens (activities). The tool implements two exploration strategies based on this graph, a simple DFS, and targeted exploration.  ACTEve \cite{Anand:FSE12} is a  concolic-based testing approach for smartphone apps that symbolically tracks events from the point where they originate to the point where they are handled. The tool is similar in efficacy to concolic testing while avoiding the path-explosion problem, but requires Soot for instrumentation \cite{soot}. 

%\textbf{MobiGUItar }\cite{} This approach is the evolution of AndroidRipper and furthers the previous approach by more precisely modeling the states of an Android app?s GUI.  This work implements a GUI "ripper" which is essentially executes feasible events in an app?s GUI hierarchy by observing and updating the current GUI state of an app in order to account for any changes in the apps GUI brought about by previous events.  MobiGUITAR uses Android ripping as a means of building a GUI state-machine model of an application. After this model is constructed, test-cases can be sampled from feasible event sequences inferred from the model using a pair-wise edge coverage criterion.

%\textbf{A$^3$E Targeted }\cite{} This is the teargeted version of the A$^3$E tool that leverages a static transition model, extracted using the SCANDroid tool \cite{}, and uses this model to more effectively explore an application's GUI.

%\textbf{Swifthand }\cite{} This approach uses machine learning to learn a model of an app and uses the learned model to generate user inputs that drive the execution of the app towards unexplored states. One of the main goals of this approach is to minimize the number of times an app under test must be restarted, as this is an expensive operation, during testing.  The main goal of the Swifthand approach is achieving high code coverage quickly. In order to achieve this the approach combines active learning with testing.  The algorithm that Swifthand employs reduces the number of restarts by heuristically exploring new screens that can be reached from the current screen without a restart.  This approach uses extended deterministic labeled transition systems (ELTS) as models for the apps GUI. 

%\textbf{QUANTUM }\cite{} This tool represents an approach for automatically generating GUI-based app-agnostic oracles for the detection of defects in Android applications.  This is a data-driven approach, based on a study of 106 bugs drawn from 13 open-source android applications, the goal of the study was to determine opportunities for automatically generating test cases that include test oracles, by focusing on bugs specific to mobile apps.  Based on the findings of the study, the authors present what they call Feature Based Testing of mobile apps.  However, the authors implemented a subset of the app-agnostic features they discerned from the study, namely rotation, killing and restarting, pausing and resuming, and back button.  In order to generate test sequences, QUANTUM receives a model of the application?s GUI as an xml file, which needs to be manually generated in the tools current iteration, and adds edges for features where the oracle testing will be applied, and generates a visual representation of the model for user verification.  Once the model is generated, the tool traverses the model and generates a suit of J-Unit test cases using a combination of Robotium and Junit to exercise events. 

%\textbf{ORBIT } \cite{} This approach uses static analysis in order to extract the set of events coupled to the GUI of a particular app, and then uses dynamic GUI crawling to construct a model of the application.  The static analysis component of this tool scans the layout files of the app and identifies the GUI components defined in these layout files, then it locates any handlers or event listeners in the source files of the application in order to extract the possible fireable actions associated with each component.  ORBIT models the GUI of an application as a finite state machine.   This tool implements two types of GUI exploration strategies, one is a traditional DFS, where, once a sate in the app is reached where no more actions can be performed, they start the app from scratch and navigating to the state (in this case screen) before the state where the exploration hit a dead end.  However, because this is somewhat expensive in terms of testing time, they perform a lightweight version of this exploration using the ?Back? button present on Android devices.

%\textbf{MonkeyLab } \cite{} Since past studies have shown that developers typically prefer manual testing over automated approaches, MonkeyLab takes a unique approach to testing, namely it implements a lightweight record-replay mechanism based on RERAN \cite{} that allows developers to record testing scenarios.  Then, the approach constructs a model using an N-Gram based NLP machine learning technique in order to generate (un)seen event sequences from user data and cover orthogonal program statements.

\textbf{Model-Based Input Generation} approaches attempt to build detailed models (e.g., capturing relevant screen and event flows) of apps in order to be able to explore them more effectively.  MobiGUItar \cite{Amalfitano:IEEE14} is the evolution of AndroidRipper and models the states of an Android app's GUI, executing feasible events by observing and updating the current GUI state of an app. %Using an stack of visited components \CrashScopebf is able to manage current GUI components and transitions require to reach the particular component without using a GUI state-machine model of an application as MobiGUItar. 
Swifthand \cite{Choi:OOPSLA13} uses active learning to infer a model of an app and uses the learned model to generate inputs that drive the execution of the app towards unexplored states. Additionally, this approach aims to minimize app restarts, due to restart overhead, by exploring all screens that can be reached from the initial state of the app first. %This approach uses extended deterministic labeled transition systems (ELTS) as models for the apps GUI, on the other hand \CrashScopebf uses a simple list of transitions triggered by specific components. 
QUANTUM \cite{Zaeem:ICST2014} represents an approach for automatically generating GUI-based app-agnostic oracles for the detection of defects in Android applications. The tool implements a set of app-agnostic features, namely: rotation, killing and restarting, pausing and resuming, and back button. It is able to present a visual representation of the app to the developer for verification after exercising the previous features at targeted locations during testing. %The testing of contextual features in \CrashScopesp were motivated in part by the study presented in \cite{ZaeemICST14}.  \CrashScopebf executes an app in differing contextual conditions by directly manipulating sensors such as Magnetometer, GPS, Network, Temperature and Accelerometer, for the purpose of exposing crashes related to these app-agnostic features. 
While QUANTUM can not produce detailed crash reports, it can produce replayable Junit/Robotium test cases. ORBIT \cite{Yang:FASE13} uses static analysis to extract GUI-components in the layout files and locate any handlers or event listeners in the source files in order to extract possible fireable actions. Then, it uses dynamic GUI crawling to construct a model of an app. MonkeyLab \cite{Linares:MSR15} is an approach that mines application usages to extract \textit{n}-grams representing the GUI and usage models.  MonkeyLab is capable of generating unseen and actionable sequences of events that achieve orthogonal code coverage compared to the application usages mined to generate the model.  Tonella et. al. \cite{Tonella:ICSE2014} also applied interpolated \textit{n}-grams to model based testing, but not in the context of mobile apps.%While \CrashScope does not extract event-handlers for specific GUI components, it does extract the locations APIs related to the contextual events listed above, allowing for targeted testing of such events only in the app Activities or screens that implement them.
%\textbf{PUMA }\cite{} This approach is a programmable framework that attempts to separate the logic required for exploring an app and the logic for analyzing an app?s properties. It accomplishes this by offering developers a generic UI automation capability that exposes high-level events for which users can define handlers.  This approach is less an automated input generation technique and instead has the goal of creating a programmable UI-Automation framework for which developers can implement their own exploration strategies.    PUMA implements a programmable UI-Automation language that supports the creation of different state exploration schemes for different goals while supporting access to the current app GUI state, GUI actions and system events.  This system instruments application binaries and uses UIAutomator to achieve its features.

%\textbf{Thor }\cite{} This is an android testing and debugging approach that relies on the existence of existing test sequences and systematically exposes them to adverse conditions.  The tool was implemented for Android apps and Robotium test suites.  Thor injects adverse conditions after each event triggered on an app, and thus it relies on the determination of neutral event sequences, those that should not contribute to a crash, meaning contextual events that complement the ordinary user UI events.  Once these neutral event sequences have been isolated, they can be injected into an application during the course of a normal UI test case, and if a test assertion fails for one of these injected events, it is safe to assume that the app is misbehaving at that particular point.  

%\textbf{AppDoctor }\cite{Hu:ESYS14}  AppDoctor \cite{Hu:ESYS14} has as its goal discovering bugs in Android apps.  This tool takes an ``approximate execution" approach to uncovering bugs within an app.  In this approach the tool uses a side loaded instrumentation app to hook directly into event handlers associated with various application GUI components and executes these handlers directly.  However, because each handler may (or may not) be user accessible it has as a consequence the possibility of reporting false positive bugs and crashes.  To rectify this problem the approach executes the ``real" actions (e.g., low-level touch events) that should trigger a bug, to confirm bugs and crashes.  While this approach does offer the ability to replay the bugs and presents the developer with stack traces, it does not offer highly detailed and expressive reports that contribute to debugging the problem at the root of a fault or crash

%\textbf{SPAG-C }\cite{}  This approach is aimed at determining whether or not a given device is capable of displaying an application that is assumed to be working correctly.  The authors focus on the accuracy efficiency and reusability of automated test oracles for Android devices, with a focus on the correctness of GUI display using a black box approach.  The authors first approach, SPAG (Smart Phone Automated GUI Testing tool) combines two open source tools: Sikuli, for UI Automation, and Android screencast for capturing the frame buffer for a device.  SPAG merges these two tools together and enables using Sikuli?s API for testing Android devices.  The main novelty of this approach is an automatic verification method that uses Android accessibility features in order to record transitions between activities after an event is executed.

%\textbf{JPF-Android }\cite{} This is a model checking tool for Android applications that allows them to verified outside of an emulator on Java PathFinder (JPF).  The major goal of this framework is to verify Android applications by running the application code on the JVM using a collection of different event sequences and then detecting when certain errors occur using JPF.  Since JPF usually uses as a target the main method of a Java program to initialize a search, and Android does not have a main method but instead relies on callback methods corresponding to specific lifecycle stages in the application.  JPF-Android uses the Main Activity as the target, and when the class corresponding to the Main activity is loaded JPF-Android a main method is injected by JPF Android, the main method starts up the entire Android software stack model and in turn starts up the entire application.  

%\textbf{\CrashDroid }\cite{} This is a previous work of the authors and a project that motivated the CrashScope approach. \CrashDroid is an approach that can translate the Call Stack from a Crash Report into expressive steps to reproduce a bug.  However, it has some limitations, namely \CrashDroid is not able to uncover Android crashes automatically, but instead relies on pre-existing stack traces, second the tool requires expensive collection of manual traces from users that need to be annotated with natural language descriptions, which are needed to construct the bug reports and replayable scenarios.

\textbf{Other Approaches in Mobile Testing and Bug Reporting} encompass emerging work that attempts to solve specific problems related to testing and bug reporting in a mobile context.  PUMA \cite{Hao:Mobisys14} exposes high-level events for which users can define handlers, in order to create a programmable UI-Automation framework for which developers can implement their own exploration strategies. This system relies on the instrumentation of app binaries and implements a basic random input generation approach.  Thor \cite{Adamsen:ISSTA2015} relies on existing test cases for an app and systematically triggers adverse contextual conditions during the execution of the sequences in given test case. %CrashScope is able to implement a similar contextual testing approach and apply it to completely automatic input generation.  
AppDoctor \cite{Hu:ESYS14} takes an ``approximate execution" approach by using a side loaded instrumentation app to hook directly into event handlers that are associated with various application GUI-components.  While this approach does offer the ability to replay the bugs and presents the developer with stack traces, it must replay crash traces to prune false-positives and it does not offer highly detailed and expressive reports as \CrashScopesp does. SIG-Droid~\cite{Mirzaei:ISSRE15} infers test inputs by relying on symbolic execution, and combining inputs with a GUI model extracted automatically from the source code. SPAG-C \cite{Lin:TSE14} is aimed at determining whether or not a given device is capable of correctly displaying an app that is assumed to be working correctly. This approach combines Sikuli, for UI Automation, and Android screencast for capturing the frame buffer of a device.  JPF-Android \cite{vanderMerwe:SEN2014} verifies Android apps by running android code on the JVM using a collection of different event sequences and then detecting when certain errors occur using Java PathFinder (JPF).  This approach introduces overhead due to the stack manipulation, listeners and logging used by JPF, and is severely limited in terms of the types of events it can properly execute. Evodroid \cite{Mahmood:FSE14} expands upon a typical systematic strategy and leverages evolutionary algorithms that use Interface and Call-Graph models. \\% in order to support the testing of apps.%; however, it is not aimed at producing expressive crash reports.%\CrashScopesp does not need any low level instruction interpreter to be executed, it can be executed on any GUI-based app.\\
\indent The motivation for \CrashScopesp stems in part from our previous work in mobile bug and crash reporting \cite{White:ICPC15,Moran:FSE15,Moran:ICSE16}.  \CrashDroid \cite{White:ICPC15} is capable of translating a call stack from an app crash into expressive steps to reproduce a bug. However, it has two noteworthy limitations: first, it is not able to uncover crashes automatically, but instead relies on pre-existing stack traces; second, the tool requires expensive collection of manual traces from real users that need to be annotated using natural language descriptions, which are needed to construct the bug reports and replayable scenarios.  FUSION \cite{Moran:FSE15,Moran:FSESRC2015,Moran:ICSE16} is a bug reporting mechanism that leverages program analysis to facilitate users creating expressive bug reports.  However, this approach requires users to create bug reports for functional problems in an app.  \CrashScopesp automates the entire crash discovery process and adds information regarding the contextual state of the app at each reproduction step, resulting in a tool that automates a typically expensive maintenance process for developers.

	%In order to identify the most prevalent causes of crashes for Android applications, and thus the features that should be included in a practical tool for automatically uncovering crashes, we conducted a qualitative study \DENYS{mention grounded theory later with a link} on 200 crash reports drawn randomly drawn from \#\# reports sampled from 149 open-source Android applications hosted on the F-Droid marketplace, the largest repository of freely available open source Android apps \cite{fdroid}.  Our goal in selecting apps for this study was to sample a diverse set of applications in order to categorize broadly applicable causes of crashes for Android applications which could in turn be directly tested in an automated fashion.  

	%We performed a keyword search for several phrases related to Android application crashes including: \textit{crash, force close, exception, forceclose, force-close, stop responding, responsive, failed, unexpected, stopped, anr ,oom, unresponsive, lags} to filter for reports that specifically discuss applications crashes. In order to ensure that the bug reports we examined had identifiable causes, we sampled only \textit{closed} reports for the set of applications.  To conduct a grounded-theory based study we split the set of 200 randomly sampled reports into two groups of 100 unique reports, and assigned one group of 100 reports to each of the authors such that every report was evaluated by two individuals.  The four authors manually examined each of the 100 reports and either discarded the report if it did not specifically relate to a crash or categorized the cause of the crash to the best of their knowledge.  After this initial round of categorization, the authors met to come to a consensus regarding the categorizations of the causes of each crash.  the results of the consensus reached are outlined in Table \ref{crash-report-results}.
	
	
\vspace{-0.15cm}
\subsection{Previous Studies on Mobile App Bug/Crashes}
\vspace{-0.1cm}
	Motivating factors from mobile app bug/crash studies aided us in designing \CrashScope. Two studies stand out in terms of providing information to drive design decisions for our approach. First, Ravindranath \emph{et al.} \cite{Ravindranath:Mobisys2014} conducted a study of 25 million real-world crash reports collected from Windows Phone users ``in the wild" by the ``Windows Phone Error Reporting System" (WPER).  Although this study was conducted regarding crashes from a different mobile OS, several of the findings reported in this study are relevant in the context of Android, due to platform similarities: 1) a small number of root causes cover a majority of the crashes examined;  2) many crashes can be mapped to well-defined externally inducible faults, for example, HTTP errors caused by network connectivity issues;  3) the dominant root causes can affect many different user execution paths in an app.  The most salient piece of information that can be gleaned from the study and applied in the design of \CrashScopesp is the following: \textit{An effective crash discovery tool must be able to test different contextual states in a targeted manner, while remaining resilient to encountered crashes so as to uncover crashes present in different program event-sequence paths.} We explain how \CrashScopesp achieves targeted testing of contextual states using program analysis in Sec. \ref{sec:approach}.
	
	In addition, Zaeem \emph{et al.} \cite{Zaeem:ICST2014} conducted a bug study on 106 bugs drawn from 13 open-source Android applications, with the goal of identifying opportunities for automatically generating test cases that include oracles. %While this study does not specifically examine bug crashes, the authors note some interesting findings that helped to inform the design of \CrashScope.  
Most notably, the results of this study were formulated as a categorization of different Android app bugs.  Specifically, these categorizations were grouped into three headings: Basic Oracles, App-Agnostic Oracles, and App-Specific Oracles.  \CrashScopesp uses the well-defined oracles of uncaught exceptions and app crashes to detect faults; however, some of the bug categorizations in this study are useful in triggering these, specifically the app-agnostic categorizations of \textit{Rotation}, \textit{Activity Life-Cycle}, and \textit{Gestures}.  Specifically, we implemented a targeted (i.e. localized) version of the double-rotation feature \cite{Zaeem:ICST2014}.

%\DENYS{there are other strategies, not only random. Also, why quotes for random?} 
%\cite{Machiry:FSE13}. \textit{GUIRipper} \cite{Amalfitano:ASE12} and \textit{MobiGUITAR} \cite{Amalfitano:IEEE14} are systematic strategies that dynamically build a model of the app under test and implement a Depth-First-Search (DFS) strategy, where the application is restarted when new states are no longer discovered.  \textit{A}$^3$\textit{E} \cite{Azim:OOPSLA13} is another tool that implements a systematic exploration based on DFS, but has the added feature of leveraging a high-level control flow graph containing the allowed transitions between activities.  \textit{Swifthand} \cite{Choi:OOPSLA13} is a tool that uses machine learning to derive a model of an Android app in order to explore unvisited states and minimize the need to restart the app.  \textit{EvoDroid} \cite{Mahmood:FSE14} is an approach that relies on evolutionary algorithms to generate inputs where the fitness function is intended to maximize the code coverage of the app under test. \textit{ACTEve} \cite{Anand:FSE12} is a concolic testing tool that symbolically tracks concrete events as they are executed on an app, checks for subsumption in event sequences and requires instrumentation of both the system and the app under test. \textit{MonkeyLab} \cite{Linares:MSR15} is a recent approach that employs a lightweight collection of users traces upon which it learns a statistical language model of app usages. The tool can then generate inputs in either a serial or online mode in which (un)natural input sequences can be provided by the language model.  Nguyen et al. developed a model-based system for testing GUI-based applications based on an \textit{observe $\rightarrow$ model $\rightarrow$ execute} paradigm \cite{Nguyen:TSE14}
	
\begin{figure*}[tb]
\vspace{-0.9cm}
\centering
\includegraphics[width=\linewidth]{img/CrashScope_Design_ICST.pdf}
\vspace{-0.7cm}
\caption{Overview of CrashScope Workflow}
\label{Design}
\vspace{-0.7cm}
\end{figure*}
	
	
%\subsection{Limitations of Current Mobile Automated Testing Approaches}
\vspace{-0.15cm}
\subsection{Limitations of Mobile Testing Approaches}
\vspace{-0.1cm}
\label{subsec:limitations}

	%While we have shown automatic android testing and input generation has been an active area of study in the mobile and software engineering research community.  However, 
	While significant progress has been made in the area of testing and automatically generating inputs for mobile applications, the available tools generally exhibit some noteworthy limitations that inspired the development of \CrashScope:
	
\begin{itemize}
\item{Previous approaches lack the ability to provide detailed, easy-to-understand testing results %\MARIO{\textcolor{red}{THis is a big claim. Please do not confuse debugging with testing. Debugging includes variables and app state. Crashscope does not provide that. I would change detailed debugging with "reproduction steps"}}
for faults discovered during automatic input generation, leaving the developer to sort through and comprehend stack traces, log files, and non-expressive event sequences \cite{Choudhary:ASE15}};
\item{Most approaches for automated input generation are not practical for developers to use, typically due to instrumentation or difficult setup procedures.  This is affirmed by the fact developers typically prefer manual over automated testing approaches \cite{Kochhar:ICST15,23Joorabchi:ESE13,Linares:ICSME15}}. As we show, instrumentation can contribute to a higher than necessary developer effort in parsing results from automated approaches, because developers must sift through ``false positive" crashes caused by instrumentation. %\MARIO{I do not understand the purpose of the last senence. I do not see the connection between instrumentation, developer effort, and parsing results};
\item{Few approaches combine different strategies and features for testing apps through supporting different methodologies for user text input and testing of contextual states (e.g., wifi on/off) in a single holistic approach.}
\end{itemize}

These shortcomings contribute to the low adoption rate of automated testing approaches by mobile developers. In the next section of this paper, we clearly describe how \CrashScopes design addresses these current limitations in automated mobile input generation and testing tools.
  
	%Recent work surveying the current state of research in Android input generation tools has corroborated the limitations of existing approaches \cite{Choudhary:ASE15}. This study performed by Choudhary \emph{et al.} demonstrated that when using execution time as the common metric, most state-of-the-art input generation tools fail to outperform Android Monkey in metrics such as code coverage and fault discovery.  Furthermore, the authors specifically noted that most current test input generation tools lack the ability to provide detailed testing results %\MARIO{\textcolor{red}{Again. Debugging is different from testing}}
%or generate reproducible test cases of the input scenarios.  Recent work conducted by Kochhar \emph{et al.}~\cite{Kochhar:ICST15} investigated the use of test cases and automated testing tools by open-source Android developers and found that only 14\% of apps contain test cases and only 9\% of these apps have test cases that achieve more than 40\% code coverage.  They also conducted a survey revealing that \textit{time constraints}, \textit{compatibility issues} and \textit{cumbersome tools} are three of the top four challenges faced during testing by developers.
	
	%Another study conducted by Joorabchi \emph{et al.}~\cite{23Joorabchi:ESE13} investigated the challenges that mobile app developers face, through interviews with senior mobile software developers as well as a wider survey.  %They found general challenges that include \textit{platform fragmentation}, \textit{lack of monitoring, analysis and testing support}, and \textit{keeping up with frequent platform changes}.   
%When investigating current testing practices for mobile apps they found that \textit{manual testing is prevalent}, \textit{automating GUI testing} is difficult and \textit{handling crashes} is also challenging. These findings further motivate the need for an easy to use system that can be run in a completely automatic fashion in order to support developers uncovering and reporting bugs in their application before release.  We conjecture that if developers had access to a practical fault detection tool for mobile apps, such as \CrashScope, which could be run in the background and is compatible with several popular versions of the Android platform, it would greatly improve the current landscape of testing and the challenges listed above, while consequently improving the quality of mobile applications.  
	
		%In addition, \CrashScopesp also addresses some limitations of these previous approaches which highlight the practicality of our tool.
%For instance, our approach is completely black-box, requiring no instrumentation of the system or app source code, making it incredibly easy to operate.  This means \CrashScopesp supports \textit{both} emulators and physical devices running popular versions of the Android OS that support the \texttt{UIAutomator} subroutines (version 4.3+), upon which our implementation is based.  The ability to operate on \textit{both} actual devices as well as emulators is important, as many apps are tested directly on devices from with different specifications, versions of Android, and screen sizes, and is a major challenge in app development\cite{23Joorabchi:ESE13}  Our approach is capable of detecting a crash during execution, logging the information for that fault and continuing with execution of the app, meaning CrashScope is fault tolerant.  
%\subsection{Mobile Bug Detection and Reporting}

%	There are a limited number of studies specifically looking into the problem of discovering and reporting Android app crashes.  We take as motivation previous work on \CrashDroid aimed at generating reproducible bug reports from Android app crashes \cite{White:ICPC15}, however, \CrashDroid has a few key limitations.  First, \CrashDroid is not able to uncover Android crashes automatically, but instead relies on pre-existing stack traces, second the tool requires expensive collection of manual traces from users that need to be annotated with natural language descriptions, which are needed to construct the bug reports and replayable scenarios.  \CrashScopesp addresses these limitations by 1) offering a systematic exploration strategy that can automatically explore an app's GUI layout and uncover crashes; 2) using information extracted from GUI components at runtime to automatically create detailed bug reports and high-level, human readable, and portable scripts that can be replayed on device(s) or emulator(s).    
	
%	Another closely related work is AppDoctor \cite{Hu:ESYS14}, which has as its goal discovering bugs in Android apps.  This tool takes an ``approximate execution" approach to uncovering bugs within an app.  In this approach the tool uses a side loaded instrumentation app to hook directly into event handlers associated with various application GUI components and executes these handlers directly.  However, because each handler may (or may not) be user accessible it has as a consequence the possibility of reporting false positive bugs and crashes.  To rectify this problem the approach executes the ``real" actions (e.g., low-level touch events) that should trigger a bug, to confirm bugs and crashes.  While this approach does offer the ability to replay the bugs and presents the developer with stack traces, it does not offer highly detailed and expressive reports that contribute to debugging the problem at the root of a fault or crash, while \CrashScopesp does.  \CrashScopesp also does not require any instrumentation to be added to an app, and conversely to AppDoctor, \CrashScopesp relies on \textit{concrete} app execution to detect crashes, instead of approximate execution, eliminating the possibility of false positives.  Hu and Iulian \cite{Hu:AST11} describe a framework for finding GUI bugs in Android apps involving instrumentation of the VM and post-processing the log files, however, this approach does not produce replayable scenarios or produce bug reports for the faults.  Ravindranath \emph{et. al.} developed VanarSena \cite{Ravindranath:Mobisys14}, a framework for testing windows phone apps on the cloud and reporting crashes and failures, and while their framework reports faults and crashes it does not provide detailed bug reports with reproduction steps or replayable scenarios that will reproduce the fault or crash.  

\begin{comment}	
\begin{table}[b]
\centering
\caption{Results of Crash Categories for Android Application Crashes}
\label{fig:android_approaches}
\scriptsize

\begin{tabular}{ | p{65pt}  | l | l | l | l | }
\hline
	 & Cat 1 & Cat 2 & Cat 3 & Cat 4 \\ \hline
	\# of Crash Reports Related to Category &  &  &  &  \\ \hline
\end{tabular}
\end{table}
\end{comment}
	

==> results.tex <==
\subsection{Results for Empirical Study 1}

\begin{table*}[tb]
\centering
\small
\caption{Summary of the crashes and exceptions uncovered for each tool.}
\label{tab:crash-results}
\vspace{-0.5cm}
\end{table*}


\subsection{Results for Empirical Study 2}

\KEVIN{TODO: Insert table summarizing the results of Bug reproduction study}

\subsection{Discussion}

Here we will discuss any interesting results from either study.  We specifically want to highlight cases where \CrashScope is better than the other tools at detecting crashes and exceptions.

==> study.tex <==
% !TEX root = main.tex
To evaluate \CrashScopesp we performed two empirical studies:  one focused on evaluating the fault finding capabilities of \CrashScope, and the other aimed at evaluating the accuracy and usefulness of the reports generated by \CrashScope.  
%We outline the design and methodology of these studies below.

\subsection{Empirical Study 1: Evaluating the Fault Discovery Capabilities of CrashScope}

 The \textit{goal} of the first study is to evaluate the effectiveness of \CrashScope at discovering bugs in Android applications with \textit{purpose} of improving automated techniques for uncovering and reporting bugs in mobile applications.  The \textit{quality focus} of this first study concerns the fault detection capabilities of \CrashScope in terms of locating exceptions and crashes in Android applications.  The \textit{context} of this study consists of the 5 state-of-the-art automated input generation tools for Android listed in Table \ref{tool-table}, 68 open-source Android applications available on the F-Droid marketplace \cite{fdroid}, and Android Nexus 5 and Nexus 7 devices as well as Android emulators running various OS versions.  
 
 \begin{table}[t]
 \centering
  \caption{Tools used in the comparative fault finding study}
 \label{tool-table}
 \begin{adjustbox}{width=\columnwidth}
 \begin{tabular}{  c | c | c }
  \hline                       
  Tool Name & Tool Type & Android Version \\ \hline
  Monkey & Random & any \\
  A$^3$E Depth-First & Model-Based & any \\
  ACTEve & Systematic & v2.3 \\ 
  GUIRipper & Model-Based & any \\
  Dynodroid & Random-Based & v2.3 \\
  Swifthand & Model-Based & v4.1+ \\
  \hline  
\end{tabular}
\end{adjustbox}
\end{table}

\subsubsection{Research Questions}

The first study aimed at empirically determining how well, compared to other approaches, \CrashScope is able to detect failures in Android applications.  To this end, we examined the following research questions:

\begin{itemize}
\item{\textbf{RQ$_1$}: \textit{Is CrashScope able to detect more application exceptions or crashes as compared to the other automated input generation tools?}} \DENYS{I would rather put it How does CrashScope compare to other automated input generation tools in terms of detecting app exceptions and crashes?}
\item{\textbf{RQ$_2$}: \textit{Is CrashScope able to better detect a particular type of crash or exception better than the other tools?}}\DENYS{I agree - this question can go as it does not contribute drastically to the main message, unless we have some super interesting results that we can clearly explain}
\item{\textbf{RQ$_3$}: \textit{Are some CrashScope execution strategies more effective at uncovering exceptions and faults than others?}}
\item{\textbf{RQ$_4$}: \textit{Is CrashScope able to discover different bugs across different devices or OS versions?}}

\end{itemize}
\MARIO{I do not like the last one in particular because of the "different OS versions". Think about the following "are testers able of detect bugs across different devices or OS versions?". For sure, they just have to test the app in a different device. Can the other apps do the same? Maybe yes or maybe not. If not, this is an implementation issue but not an approach issue. So, IMHO this does not deserve a RQ, but must be analyzed as part of one of the other RQs. Detecting bugs in different versions/devices  is a feature of  CrashScope derived of the fact that the replayable scripts are at GUI -level. By the way, the approach needs to mention that the idea of high-level scripts is inspired in MonkeyLab}

\subsubsection{Methodology}

	In order to compare \CrashScopesp against other state of the art automated input generation tools for Android we utilized the set of Subject Apps and tools available in the Androtest testing suite \cite{Choudhary:ARCX15}.  We ran the tools listed in Table \ref{tool-table} using Vagrant and VirtualBox \DENYS{add refs to Vagrant and VirtualBox} as described in the authors online instructions \cite{androtest-online}.  Each tool was allowed to run for one hour for each of the 68 subject applications, except Dynodroid and Monkey, which were run 10 times due to non-deterministic nature of those tools. \MARIO{Are you sure swifthand is deterministic? Swifthand uses active learning, which can be non-deterministic}  The Androtest suite allows for multiple instances of virtual machines containing the tools to be spawned and run concurrently. Each tool ran on its required Android version or Android version 19 KitKat.  Since the \textit{goal} of this study is to determine the exception and crash discovery capability of each of the tools, we wrote a script to automatically parse exceptions from the \texttt{logcat} that is returned by each tools execution.  We classified both exceptions that directly led to an application crash, as well as "silent exceptions"\MARIO{what is a silent exception? The right term is caught exception or handled exception} that allowed for the continued execution of the application by the tool.  
	
	In order to compare \CrashScopesp against these tools, we extracted an recompiled the 68 subject Android apps from the testing suite so that they could be installed on a physical Android device upon which \CrashScopesp would operate.  During this study we ran each \CrashScopesp strategy on a Nexus 5 phone and Nexus 7 tablet, two times with different versions of the Android OS installed (v4.4.2 \& v5.0.1).  We chose to run \CrashScopesp across different devices and operating system versions to see what impact if any different hardware, or API version levels had on the ability of \CrashScopesp to uncover exceptions and crashes in the subject apps.  The details of the subject applications as well as the .apk files used for testing \CrashScopesp can be found in our online appendix \KEVIN{Add reference to online appendix}.  The apps from the Androtest suite include instrumentation with the Emma framework for collecting code coverage data, however, we were unsuccessful at getting some of these instrumented applications to run on our physical devices, and therefore, recompiled the failing apps without the instrumentation included.  In total, 32 of the 64 apps had to be recompiled without instrumentation to run on our devices.  
	
	To answer {\textbf{RQ$_1$} \& {\textbf{RQ$_3$} we examined the total number of unique exceptions and crashes uncovered by each tool and by each strategy of \CrashScope.  We extracted unique failures by parsing the collected stack traces for each tool and app by removing the pids and other unique information, and performing a \texttt{diff} analysis, keeping only the remaining unique stack traces.  In this experiment the more unique exceptions (including the stack trace) and crashes a tool uncovered, the better its fault detection capabilities.  To answer {\textbf{RQ$_2$} we extracted the cause of each failure in order to determine if different tools were better at detecting certain types of faults than others.  We accomplished this by parsing the first line of each stack trace and extracting the error that caused the fault \MARIO{Here we have an issue. The first line has the last reported exception, but this it not necessarily the cause of the failure}.  To answer {\textbf{RQ$_4$} we report on instances where \CrashScopesp uncovered different unique exceptions \MARIO{Please be careful. An exception is not the same that a Stack Trace. So do you mean exceptions or stack traces?} or crashes for the same apps across different devices or OS versions, and examine a few cases in order to determine the causes of such faults. 

\subsection{Empirical Study 2: Evaluating the Accuracy and Readability of \CrashScopesp Reports}

	The \textit{goal} of the second study is to evaluate the \textit{accuracy} and \textit{readability} \DENYS{and reproducibility, right?} of the natural language reports generated by \CrashScopesp with the \textit{purpose} of improving the quality of crash and exception reports provided to Android developers.  The \textit{quality focus} of this study concerns the ability of developers to reproduce bugs from \CrashScopesp reports.  The \textit{context} of this study consists of eight real world Android app crashes, extracted from apps in the F-Droid open-source repository and their corresponding issue tracker entries, as well as reports generated by \CrashScopesp for these same crashes.  This evaluation encompassed a user study involving eight graduate students from the Department of Computer Science at W\&M.  
	
	\begin{table}[h!]
\centering
\caption{Summary of bug reports used in the second study}
\label{tab:crashes}
\vspace{-0.2cm}
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{ | c | c | c | c |}
\hline
\textbf{App} & \textbf{App Version} & \textbf{Issue ID} & \textbf{Min \#steps} \\ \hline
Adsdroid & v1.5 & 7 &  3\\ \hline
Angram-Solver & v2.2 & 2 & 3\\ \hline
BMI & v1.0 & 2 & 5 \\ \hline
Eyecam & v1.0 & 22 & 3\\ \hline
GNUCash & v1.0.3 & 47 & 5\\ \hline
Olam & v1.0 & 2 & 3 \\ \hline
31C3 Scheduler & v1.30.2 & 82 & 5  \\ \hline
Card Game Scores & v1.0 & 10 & 5 \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

	
\subsubsection{Research Questions}

	Our second study aimed at empirically determining the level of \textit{accuracy} and \textit{readability} of \CrashScopes automatically generated reports compared to the original human written reports in the open source issue trackers through a user study. \MARIO{This subsection does not explain how the accuracy or the readability are measured. What metrics/questions/etc are related to accuracy/readability?} To this end we examined the following research questions:
\MARIO{Please continue the numbering from previous RQs to avoid confussions}	
\begin{itemize}
\item{\textbf{RQ$_1$}: \textit{What information (if any) is useful to developers/testers in the CrashScope bug reports?}}
\item{\textbf{RQ$_2$}: \textit{Are developers able to reproduce more bugs using CrashScope reports than with human written reports?}}
\item{\textbf{RQ$_3$}: \textit{Are developers able to reproduce bugs more quickly using reports generated by CrashScope compared to traditional human written reports?}}
\item{\textbf{RQ$_4$}: \textit{Are reports generated by CrashScope more readable than traditional human written reports?}}
\end{itemize}
\MARIO{RQ2 and RQ3 can be the same RQ}
\subsubsection{Methodology}

	In order to evaluate \CrashScopes automatically generated reports we compared them against eight human written crash reports from issue trackers of eight different apps on the F-Droid marketplace (See Table \ref{tab:crashes}) in the context of a reproduction task.  To find the crashes, we manually inspected the issue trackers of the apps on F-droid for reports that described an application crash, then we ran \CrashScope on the version of the app that the crash was reported against, to observe wether or not \CrashScope was able to capture the crash on the Nexus 7 tablet running Android 4.4.2 KitKat that would be used for reproduction user study.  While we hand-pick these bugs, the goal of this study is not to measure \CrashScopes effectiveness at discovering bugs, the previous study aims to accomplish this goal.  We willingly acknowledge that there are situations in which CrashScope will not be able to uncover a fault and we outline these cases in Section \ref{sec:limitations}.
	
	In order to answer the research questions stated above we tasked eight graduate students (considered of as developers) with the task of reproducing eight crashes (four from the original human written reports, and four from \CrashScope).  The design matrix of this study was devised in such as way that each crash for each type of report was evaluated by four participants, no crash was evaluated twice for the same participant, and four participants saw the human written reports first, and four participants saw the \CrashScope reports first, all in the interest of reducing bias toward one system. The systems names were also anonymized (\CrashScopesp to "System A" and the human written reports to "System B") as to further avoid bias.  The full design matrix can be found in our online appendix \KEVIN{Insert reference to online appendix}\DENYS{We should show design matrix in the paper if we have space}.  During the study, participants recorded the time it took them to reproduce the crash on the Nexus 7 for each report, with a time limit of ten minutes for reproduction.  If a participant could not reproduce the bug within the ten minute time frame, or gave up in trying to reproduce the bug, that bug was marked as not-reproducible for that participant.  Collecting this data allows us to answer  {\textbf{RQ$_2$} \& {\textbf{RQ$3$}.  
	
	After the completion of the crash reproduction, we had each participant fill out a brief survey, answering questions regarding the \textit{user preferences} and \textit{usability} for each type of bug report.  We also collected information about each participants programming experience and familiarity with the Android platform.  The \textit{user preference} questions were formulated based on the user experience honeycomb originally developed by Peter Moville \cite{Morville:04} and were posed to participants as  free form text entry questions as follows:
\DENYS{Do not just present these questions as we do not have space. Present them in the context of the results, especially those with the Likert scale answers. For free-form, you can highlight some sample responses for the questions in qualitative discussion}	
\begin{itemize}
\item{\textit{What information from this type of bug report did you find useful for reproducing a crash?}}
\item{\textit{What other information (if any) would you like to see in this type of bug report?}}
\item{\textit{What elements do you like most from this type of bug report?}}
\item{\textit{What elements do you like least from this type of bug report?}}
\end{itemize}

The \textit{usability} questions were created using statements based on the SUS usability scale by John Brooke \cite{Brooke:96} and were posed to participants in the form of a 5 point Likert Scale as follows:

\begin{itemize}
\item{\textit{I think I would like to have this type of bug report frequently.}}
\item{\textit{I found this type of bug report unnecessarily complex.}}
\item{\textit{I thought this type of bug report was easy to read/understand.}}
\item{\textit{I found this type of bug report very cumbersome to read.}}
\item{\textit{I thought the bug report was really useful for reproducing the crash.}}
\end{itemize}
	
	The questions regarding programming experience are based on the programming experience questionnaire developed by Feigenspan et al \cite{Feigenspan:ICPC12} and were presented to the participants as follows:
	
\begin{itemize}
\item{\textit{On a scale of 1 to 10 how do you estimate your programming experience ? (1: very inexperienced 10: very experienced)}}
\item{\textit{How experienced are you with Android programming paradigms? (1: very inexperienced 10: very experienced)}}
\item{\textit{For how many years have you been programming?}}
\item{\textit{How many years have you been studying computer science?}}
\item{\textit{How many courses did you take in which you had to implement source code?}}
\item{\textit{Have you ever had to use a bug report to resolve a problem in source code?}}
\end{itemize}
	
The qualitative and quantitative answers provided to these \MARIO{which questions? The last 6?} questions form the basis for answering \textbf{RQ$1$} \& \textbf{RQ$4$}.
	
	
	\begin{comment}
\begin{table}[tb]
\centering
\caption{\textbf{Crashes and Exceptions Found by Dynodroid, Monkey and CrashScope:} (E=Exception that did not cause crash, C=Exception that did cause crash) The various flavors of CrashScope are enumerated as follows: \textit{\textbf{A)}} Nexus 7, In-Order, v4.4.2; \textit{\textbf{B)}} Nexus 7, Reverse-Order, v4.4.2; \textit{\textbf{C)}} Nexus 7, In-Order, v5.0.1; \textit{\textbf{D)}} Nexus 7, Reverse-Order, v5.0.1}
\label{tab:fault-results}
\begin{tabular}{lllllllllllll}
\hline
\multicolumn{1}{|l|}{Application Name} & \multicolumn{1}{l}{Dynodroid}  & \multicolumn{1}{l|}{}  & \multicolumn{1}{l}{Monkey}  & \multicolumn{1}{l|}{}       & \multicolumn{1}{l}{CrashScope A} & \multicolumn{1}{l|}{}        & \multicolumn{1}{l}{CrashScope B} & \multicolumn{1}{l|}{}        & \multicolumn{1}{l}{CrashScope C} & \multicolumn{1}{l|}{}        & \multicolumn{1}{l}{CrashScope D} & \multicolumn{1}{l|}{}        \\ \hline
\multicolumn{1}{|l|}{}           & \multicolumn{1}{l|}{E} & \multicolumn{1}{l|}{C} & \multicolumn{1}{l|}{E} & \multicolumn{1}{l|}{C} & \multicolumn{1}{l|}{E}   & \multicolumn{1}{l|}{C} & \multicolumn{1}{l|}{E}   & \multicolumn{1}{l|}{C} & \multicolumn{1}{l|}{E}   & \multicolumn{1}{l|}{C} & \multicolumn{1}{l|}{E}   & \multicolumn{1}{l|}{C} \\ \hline
\multicolumn{1}{|l|}{a2dpvol}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{4}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{aagtl}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{2}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{aarddict}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{aCal}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{adsdroid}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{AlarmClock}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{Blokish}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{Dialer}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{hndroid}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{Jamendo}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{Nectroid}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{PasswordMakerPro}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{Photostream}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{3}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{QuickSettings}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{RandomMusicPlayer}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{3}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{Soundboard}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{SyncMyPix}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{Wikipedia}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\multicolumn{1}{|l|}{Yahtzee}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} &\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{1}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-}&\multicolumn{1}{l|}{-} \\ \hline
\end{tabular}
\end{table}
\end{comment}



